Automatic Evaluation of Generative Models with Instruction Tuning

Automatic evaluation of natural language generation has long been an elusive goal in NLP.A recent paradigm fine-tunes pre-trained language models to emulate human judgements for a particular task and evaluation criterion. Inspired by the generalization ability of instruction-tuned models, we propose a learned metric based on instruction tuning. To test our approach, we collected HEAP, a dataset of human judgements across various NLG tasks and evaluation criteria. Our findings demonstrate that instruction tuning language models on HEAP yields good performance on many evaluation tasks, though some criteria are less trivial to learn than others. Further, jointly training on multiple tasks can yield additional performance improvements, which can be beneficial for future tasks with little to no human annotated data.

==> backup/results_cluster1.tex <==
\begin{table}
\centering
\begin{tabular}{p{0.1\linewidth}p{0.25\linewidth}p{0.25\linewidth}p{0.25\linewidth}}
\hline
\textbf{Task} & \textbf{Accuracy} & \textbf{Pearson's Correlation} & \textbf{Spearman's Correlation}\\
\hline


AH
                        & $56.39 \pm 2.08$
                        & $n/a$
                        & $n/a$
                        \\

AV   
                        & $53.9 \pm 1.00$
                        & $0.063$
                        & $0.043$
                        \\

QA
                        & $52.78 \pm 5.79$
                        & $na$
                        & $na$
                        \\

HS
                        & $44.46 \pm 0.44$
                        & $na$
                        & $na$
                        \\
                        
CR
                        & $48.77 \pm 1.90$
                        & $na$
                        & $na$
                        \\

BCN
                        & $58.00 \pm 2.16$
                        & $na$
                        & $na$
                        \\

SRC
                        & $41.53 \pm 4.70$
                        & $na$
                        & $na$
                        \\

DIA
                        & $43.86 \pm 2.57$
                        & $-0.101$
                        & $-0.097$
                        \\

DII
                        & $50.61 \pm 4.45$
                        & $-0.016$
                        & $-0.001$
                        \\


\hline

\end{tabular}
\begin{tabular}{lc}
\hline
\end{tabular}
\caption{Cluster: Advice Helpfullness, Answer Validity, Question Answerability, HellaSwag, Commonsense Reasoning, Best CN, Story Rewriting Counterfactual, Defeasible Inference Attenuator, Defeasible Inference Effectiveness}
\label{table:tasks}
\end{table}

==> backup/results_cluster2.tex <==
\begin{table}
\centering
\begin{tabular}{p{0.1\linewidth}p{0.25\linewidth}p{0.25\linewidth}p{0.25\linewidth}}
\hline
\textbf{Task} & \textbf{Accuracy} & \textbf{Pearson's Correlation} & \textbf{Spearman's Correlation}\\
\hline


AH
                        & $52.22 \pm 6.14$
                        & $n/a$
                        & $n/a$
                        \\

AV   
                        & $50.36 \pm 6.14$
                        & $-0.042$
                        & $-0.027$
                        \\

QA
                        & $43.58 \pm 6.30$
                        & $na$
                        & $na$
                        \\

                        
CR
                        & $35.20 \pm 2.42$
                        & $na$
                        & $na$
                        \\

BCN
                        & $54.00 \pm 0.00$
                        & $na$
                        & $na$
                        \\

SRC
                        & $52.46 \pm 5.91$
                        & $na$
                        & $na$
                        \\

DIA
                        & $56.02 \pm 0.65$
                        & $0.059$
                        & $0.085$
                        \\

DII
                        & $49.79 \pm 4.53$
                        & $-0.010$
                        & $0.024$
                        \\


\hline

\end{tabular}
\begin{tabular}{lc}
\hline
\end{tabular}
\caption{Cluster: Advice Helpfullness, Answer Validity, Question Answerability, Commonsense Reasoning, Best CN, Story Rewriting Counterfactual, Defeasible Inference Attenuator, Defeasible Inference Effectiveness}
\label{table:tasks}
\end{table}

























\begin{table}
\centering
\begin{tabular}{p{0.1\linewidth}p{0.25\linewidth}p{0.25\linewidth}p{0.25\linewidth}}
\hline
\textbf{Task} & \textbf{Accuracy} & \textbf{Pearson's Correlation} & \textbf{Spearman's Correlation}\\
\hline




AG   
                        & $65.81 \pm 8.46$
                        & $0.071$
                        & $0.074$
                        \\

CNG
                        & $56.32 \pm 1.63$
                        & $0.168$
                        & $0.136$
                        \\

CNSp
                        & $51.17 \pm 1.49$
                        & $-0.01$
                        & $0.023$
                        \\
                        
CNSu
                        & $54.96 \pm 3.04$
                        & $0.081$
                        & $0.091$
                        \\

CNI
                        & $54.85 \pm 5.31$
                        & $-0.099$
                        & $-0.093$
                        \\

CNO
                        & $43.96 \pm 3.62$
                        & $-0.097$
                        & $-0.081$
                        \\

CNSt
                        & $65.75 \pm 3.87$
                        & $0.139$
                        & $0.166$
                        \\

HSO
                        & $58.06 \pm 3.48$
                        & $0.160$
                        & $0.163$
                        \\

SRPl
                        & $47.83 \pm 1.18$
                        & $n/a$
                        & $n/a$
                        \\

SRPr
                        & $58.00 \pm 5.89$
                        & $n/a$
                        & $n/a$
                        \\

\hline

\end{tabular}

\begin{tabular}{lc}
\hline
\end{tabular}
\caption{Cluster: AnswerGrammaticalityDataLoader, CounterNarrativeGrammaticalityDataLoader, CounterNarrativeSpecificityDataLoader, CounterNarrativeSuitabilityDataLoader, CounterNarrativeInformativenessDataLoader, CounterNarrativeOffensivenessDataLoader, CounterNarrativeStanceDataLoader, HateSpeechOffensivenessDataLoader, CounterfactualStoryRewritingPlotDataLoader, CounterfactualStoryRewritingPremiseDataLoader, CounterfactualStoryRewritingSecondDataLoader}
\label{table:tasks}
\end{table}


==> backup/results_cluster3.tex <==
\begin{table}
\centering
\begin{tabular}{p{0.1\linewidth}p{0.25\linewidth}p{0.25\linewidth}p{0.25\linewidth}}
\hline
\textbf{Task} & \textbf{Accuracy} & \textbf{Pearson's Correlation} & \textbf{Spearman's Correlation}\\
\hline




BCN
                        & $72.00 \pm 2.45$
                        & $n/a$
                        & $n/a$
                        \\

CCN   
                        & $68.54 \pm 4.00$
                        & $n/a$
                        & $n/a$
                        \\

CNG
                        & $62.84 \pm 1.08$
                        & $0.278$
                        & $0.245$
                        \\

CNSp
                        & $61.99 \pm 1.80$
                        & $0.219$
                        & $0.202$
                        \\
                        
CNSu
                        & $63.06 \pm 1.27$
                        & $0.287$
                        & $0.303$
                        \\

CNI
                        & $64.98 \pm 2.60$
                        & $0.165$
                        & $0.156$
                        \\

CNSt
                        & $68.95 \pm 3.42$
                        & $0.175$
                        & $0.113$
                        \\

HSO
                        & $53.20 \pm 1.72$
                        & $0.063$
                        & $0.082$
                        \\



\hline

\end{tabular}
\begin{tabular}{lc}
\hline
\end{tabular}
\caption{Cluster: Best CN, CHO CN, CounterNarrativeGrammaticalityDataLoader, CounterNarrativeSpecificityDataLoader, CounterNarrativeSuitabilityDataLoader, CounterNarrativeInformativenessDataLoader, CounterNarrativeStanceDataLoader, HateSpeechOffensivenessDataLoader}
\label{table:tasks}
\end{table}

==> backup/results_cluster4.tex <==
\begin{table}
\centering
\begin{tabular}{p{0.1\linewidth}p{0.25\linewidth}p{0.25\linewidth}p{0.25\linewidth}}
\hline
\textbf{Task} & \textbf{Accuracy} & \textbf{Pearson's Correlation} & \textbf{Spearman's Correlation}\\
\hline



AG
                        & $49.57 \pm 6.39$
                        & $0.135$
                        & $0.130$
                        \\

AV
                        & $53.19 \pm 6.26$
                        & $-0.066$
                        & $-0.083$
                        \\

QA
                        & $43.22 \pm 2.25$
                        & $na$
                        & $na$
                        \\



\hline

\end{tabular}
\begin{tabular}{lc}
\hline
\end{tabular}
\caption{Cluster: Answer Grammaticality, Answer Validity, Question Answerability }
\label{table:tasks}
\end{table}

==> backup/results_cluster5.tex <==
\begin{table}
\centering
\begin{tabular}{p{0.1\linewidth}p{0.25\linewidth}p{0.25\linewidth}p{0.25\linewidth}}
\hline
\textbf{Task} & \textbf{Accuracy} & \textbf{Pearson's Correlation} & \textbf{Spearman's Correlation}\\
\hline



SRC
                        & $54.65 \pm 5.07$
                        \\

SRE
                        & $55.95 \pm 6.58$
                        \\

SRPl
                        & $54.59 \pm 0.68$
                        \\

SRPr
                        & $45.33 \pm 4.11$
                        \\

SRS
                        & $55.56 \pm 4.16$
                        \\

\hline

\end{tabular}
\begin{tabular}{lc}
\hline
\end{tabular}
\caption{Cluster: CounterfactualStoryRewritingCounterfactual, CounterfactualStoryRewritingEnding, Counterfactual Story Rewriting Plot }
\label{table:tasks}
\end{table}

==> backup/results_cluster6.tex <==
\begin{table}
\centering
\begin{tabular}{p{0.1\linewidth}p{0.25\linewidth}p{0.25\linewidth}p{0.25\linewidth}}
\hline
\textbf{Task} & \textbf{Accuracy} & \textbf{Pearson's Correlation} & \textbf{Spearman's Correlation}\\
\hline

DIA
                        & $67.42 \pm 3.09$
                        & $0.2755$
                        & $0.2908$
                        \\

DII
                        & $53.77 \pm 1.40$
                        & $-0.080$
                        & $-0.051$
                        \\

\hline

\end{tabular}
\begin{tabular}{lc}
\hline
\end{tabular}
\caption{Cluster: Defeasible Inference Attenuator Effectiveness, Defeasible Inference Intensifier Effectiveness}
\label{table:tasks}
\end{table}

==> backup/results_pearson.tex <==
\begin{table*}
\centering
\begin{tabular}{l | llll}
\hline
\textbf{Task} & \textbf{Base-line} & \textbf{Single-task} & \textbf{Multi-task} & \textbf{Cross-task}\\
\hline


Answer Grammaticality   & 0.093
                        & \textbf{0.394}
                        & 0.215
                        & 0.186
                        \\

Answer Validity         & 0.098
                        & -0.038
                        & \textbf{0.268}
                        & 0.095
                        \\

Counter Narrative Grammaticality
                        & 0.057
                        & 0.484
                        & \textbf{0.544}
                        & 0.188
                        \\

Counter Narrative Specificity
                        & 0.034
                        & 0.204
                        & \textbf{0.306}
                        & 0.087
                        \\
                        
Counter Narrative Suitability
                        & -0.117
                        & 0.162
                        & \textbf{0.429}
                        & -0.015
                        \\

Counter Narrative Informativeness
                        & -0.056
                        & \textbf{0.569}
                        & 0.513
                        & -0.019
                        \\

Counter Narrative Offensiveness
                        & 0.198
                        & 0.445
                        & \textbf{0.550}
                        & -0.146
                        \\

Counter Narrative Stance
                        & -0.075
                        & 0.433
                        & \textbf{0.435}
                        & 0.132
                        \\

Hate Speech Offensiveness
                        & -0.202
                        & 0.430
                        & \textbf{0.404}
                        & 0.081
                        \\

Defeasible Inference Attenuator Effectiveness
                        & -0.016
                        & 0.311
                        & \textbf{0.316}
                        & 0.263
                        \\

Defeasible Inference Intensifier Effectiveness
                        & 0.053
                        & \textbf{0.224}
                        & 0.191
                        & 0.045
                        \\





\hline
\end{tabular}
\caption{\label{results:pearsonscorrelation}
Pearson's Correlation
}
\end{table*}

==> backup/results_spearman.tex <==
\begin{table*}
\centering
\begin{tabular}{l | llll}
\hline
\textbf{Task} & \textbf{Base-line} & \textbf{Single-task} & \textbf{Multi-task} & \textbf{Cross-task}\\
\hline


Answer Grammaticality   & 0.181
                        & \textbf{0.379}
                        & 0.231
                        & 0.146
                        \\

Answer Validity         & 0.063
                        & -0.026
                        & \textbf{0.293}
                        & 0.093
                        \\

Counter Narrative Grammaticality
                        & 0.089
                        & 0.472
                        & \textbf{0.538}
                        & 0.193
                        \\

Counter Narrative Specificity
                        & 0.086
                        & 0.211
                        & \textbf{0.278}
                        & 0.090
                        \\
                        
Counter Narrative Suitability
                        & -0.152
                        & 0.143
                        & \textbf{0.413}
                        & 0.081
                        \\

Counter Narrative Informativeness
                        & -0.081
                        & \textbf{0.574}
                        & 0.472
                        & -0.014
                        \\

Counter Narrative Offensiveness
                        & 0.181
                        & 0.440
                        & \textbf{0.580}
                        & -0.125
                        \\

Counter Narrative Stance
                        & -0.087
                        & 0.436
                        & \textbf{0.461}
                        & 0.129
                        \\

Hate Speech Offensiveness
                        & -0.170
                        & \textbf{0.425}
                        & 0.399
                        & 0.086
                        \\

Defeasible Inference Attenuator Effectiveness
                        & -0.009
                        & 0.302
                        & \textbf{0.321}
                        & 0.268
                        \\

Defeasible Inference Intensifier Effectiveness
                        & 0.060
                        & \textbf{0.252}
                        & 0.215
                        & 0.080
                        \\



\hline
\end{tabular}
\caption{\label{results:spearmanscorrelation}
Spearman's Correlation
}
\end{table*}

==> figures/results_cluster_with4.tex <==
\definecolor{maroon}{cmyk}{0,0.87,0.68,0.32}

\begin{table*}
\centering
\small
\setlength{\tabcolsep}{4pt}
\begin{tabular}{lrrr|lrrr}
\toprule
\textbf{Task} & \multicolumn{1}{c}{\textbf{Single-Task}} & \multicolumn{1}{c}{\textbf{Cross All}} & \multicolumn{1}{c}{\textbf{Cross Cluster}} & \textbf{Task} & \multicolumn{1}{c}{\textbf{Single-Task}} & \multicolumn{1}{c}{\textbf{Cross All}} & \multicolumn{1}{c}{\textbf{Cross Cluster}} \\
\midrule
\rowcolor{maroon!30}
\multicolumn{4}{l}{\textbf{Cluster 1: Require understanding the context C}} & \multicolumn{4}{l}{\textbf{Cluster 3: Hate speech related tasks}} \\
\midrule
AH & \grayc{67.33$\pm$1.60} & 55.84$\pm$7.22 & \textbf{56.39$\pm$2.08} & BCN & \grayc{50.60$\pm$3.29} & 63.00$\pm$2.00 & \textbf{72.00$\pm$2.45} \\
AV & \grayc{44.35$\pm$10.03} & \textbf{58.87$\pm$10.92} & 53.9$\pm$1.00 & CCN & \grayc{64.54$\pm$12.48} & 68.16$\pm$1.72 & \textbf{68.54$\pm$4.00} \\
QA & \grayc{58.96$\pm$14.58} & 42.19$\pm$3.76  & \textbf{52.78$\pm$5.79} & CNG & \grayc{77.67$\pm$2.24} & \textbf{62.84$\pm$2.89} & \textbf{62.84$\pm$1.08} \\ 
HS & \grayc{67.91$\pm$0.42} & \textbf{51.19$\pm$0.10} & 44.46$\pm$0.44 & CNSp & \grayc{54.39$\pm$4.85} & 48.54$\pm$3.95 & \textbf{61.99$\pm$1.80} \\
CR & \grayc{77.96$\pm$4.37} & \textbf{54.32$\pm$3.86} & 48.77$\pm$1.90 & CNSu & \grayc{58.64$\pm$6.23} & \textbf{64.64$\pm$1.03} & 63.06$\pm$1.27 \\
BCN & \grayc{50.60$\pm$3.29} & \textbf{63.00$\pm$2.00} & 58.00$\pm$2.16 & CNI & \grayc{83.59$\pm$2.11} & \textbf{70.88$\pm$4.39} & 64.98$\pm$2.60 \\
SRC & \grayc{51.80$\pm$2.74} & \textbf{48.09$\pm$6.21} & 41.53$\pm$4.70 & CNSt & \grayc{76.39$\pm$2.78} & 51.60$\pm$4.18 & \textbf{68.95$\pm$3.42} \\
DIA & \grayc{65.43$\pm$6.25} & \textbf{62.03$\pm$2.29} & 43.86$\pm$2.57 & HSO & \grayc{68.81$\pm$2.94} & 49.55$\pm$0.76 & \textbf{53.20$\pm$1.72} \\
DII & \grayc{60.82$\pm$3.65} & \textbf{61.84$\pm$5.09} & 50.61$\pm$4.45 \\
\grayline
\textbf{Average} & - & 55.26 & 50.03 & 
\textbf{Average} & - & 59.90 & 64.45 \\
\midrule
\rowcolor{maroon!30} \multicolumn{4}{l}{\textbf{Cluster 2: Don't require understanding the context C}} & \multicolumn{4}{l}{\textbf{Cluster 4: Hate speech related tasks (including CNO)}} \\
\midrule
AG & \grayc{69.47$\pm$5.46} & 58.12$\pm$3.91 & \textbf{65.81$\pm$8.46} & BCN & \grayc{50.60$\pm$3.29} & 63.00$\pm$2.00 & \textbf{69.00$\pm$4.58} \\
CNG & \grayc{77.67$\pm$2.24} & \textbf{62.84$\pm$2.89} & 56.32$\pm$1.63 & CCN & \grayc{64.54$\pm$12.48} & \textbf{68.16$\pm$1.72} & 64.05$\pm$4.05 \\
CNSp & \grayc{54.39$\pm$4.85} & 48.54$\pm$3.95 & \textbf{51.17$\pm$1.49} & CNG & \grayc{77.67$\pm$2.24} & 62.84$\pm$2.89 & \textbf{63.22$\pm$4.6} \\ 
CNSu & \grayc{58.64$\pm$6.23} & \textbf{64.64$\pm$1.03} & 54.96$\pm$3.04 & CNSp & \grayc{54.39$\pm$4.85} & 48.54$\pm$3.95 & \textbf{59.36$\pm$0.51} \\
CNI & \grayc{83.59$\pm$2.11} & \textbf{70.88$\pm$4.39} & 54.85$\pm$5.31 & CNSu & \grayc{58.64$\pm$6.23} & \textbf{64.64$\pm$1.03} & \textbf{64.64$\pm$2.17} \\
CNO & \grayc{67.35$\pm$6.19} & 28.50$\pm$3.64 & \textbf{43.96$\pm$3.62} & CNI & \grayc{83.59$\pm$2.11} & \textbf{70.88$\pm$4.39} & 57.00$\pm$2.47 \\
CNSt & \grayc{76.39$\pm$2.78} & 51.60$\pm$4.18 & \textbf{65.75$\pm$3.87} & CNO & \grayc{67.35$\pm$6.19} & 28.50$\pm$3.64 & \textbf{45.38$\pm$4.68}\\
HSO & \grayc{68.81$\pm$2.94} & 49.55$\pm$0.76 & \textbf{58.06$\pm$3.48} & CNSt & \grayc{76.39$\pm$2.78} & 51.60$\pm$4.18 & \textbf{67.58$\pm$2.85} \\
SRPl & \grayc{70.72$\pm$1.21} & \textbf{50.24$\pm$6.03} & 47.83$\pm$1.18 & HSO & \grayc{68.81$\pm$2.94} & 49.55$\pm$0.76 & \textbf{52.50$\pm$1.48} \\
SRPr & \grayc{49.60$\pm$7.40} & 44.67$\pm$3.06 & \textbf{58.00$\pm$5.89} \\
\grayline
\textbf{Average} & - & 52.96 & 55.67 & \textbf{Average} & - & 56.41 & 60.30 \\
\midrule























\end{tabular}
\caption{Per-task accuracy when the model is trained on all other tasks in the cross-task setup (\textbf{Cross All}) vs. all other tasks in the same cluster (\textbf{Cross Cluster}).}
\label{tab:cluster}
\end{table*}
